Parametric Bilinear Generalized Approximate Message Passing

We propose a scheme to estimate the parameters $b_i$ and $c_j$ of the bilinear form $z_m=\sum_{i,j} b_i z_m^{(i,j)} c_j$ from noisy measurements $\{y_m\}_{m=1}^M$, where $y_m$ and $z_m$ are related through an arbitrary likelihood function and $z_m^{(i,j)}$ are known. Our scheme is based on generalized approximate message passing (G-AMP): it treats $b_i$ and $c_j$ as random variables and $z_m^{(i,j)}$ as an i.i.d.\ Gaussian 3-way tensor in order to derive a tractable simplification of the sum-product algorithm in the large-system limit. It generalizes previous instances of bilinear G-AMP, such as those that estimate matrices $\boldsymbol{B}$ and $\boldsymbol{C}$ from a noisy measurement of $\boldsymbol{Z}=\boldsymbol{BC}$, allowing the application of AMP methods to problems such as self-calibration, blind deconvolution, and matrix compressive sensing. Numerical experiments confirm the accuracy and computational efficiency of the proposed approach.

==> acknowledgement.tex <==
% use section* for acknowledgment
\section*{Acknowledgment}
The authors would like to thank Jeremy Vila for helpful discussions about EM and turbo methods for AMP. 


